HiRA: Hidden Row Activation for Reducing Refresh Latency of Off-the-Shelf DRAM Chips

DRAM is the building block of modern main memory systems. DRAM cells must be periodically refreshed to prevent data loss. Refresh operations degrade system performance by interfering with memory accesses. As DRAM chip density increases with technology node scaling, refresh operations also increase because: 1) the number of DRAM rows in a chip increases; and 2) DRAM cells need additional refresh operations to mitigate bit failures caused by RowHammer, a failure mechanism that becomes worse with technology node scaling. Thus, it is critical to enable refresh operations at low performance overhead. To this end, we propose a new operation, Hidden Row Activation (HiRA), and the HiRA Memory Controller (HiRA-MC). HiRA hides a refresh operation's latency by refreshing a row concurrently with accessing or refreshing another row within the same bank. Unlike prior works, HiRA achieves this parallelism without any modifications to off-the-shelf DRAM chips. To do so, it leverages the new observation that two rows in the same bank can be activated without data loss if the rows are connected to different charge restoration circuitry. We experimentally demonstrate on 56% real off-the-shelf DRAM chips that HiRA can reliably parallelize a DRAM row's refresh operation with refresh or activation of any of the 32% of the rows within the same bank. By doing so, HiRA reduces the overall latency of two refresh operations by 51.4%. HiRA-MC modifies the memory request scheduler to perform HiRA when a refresh operation can be performed concurrently with a memory access or another refresh. Our system-level evaluations show that HiRA-MC increases system performance by 12.6% and 3.73x as it reduces the performance degradation due to periodic refreshes and refreshes for RowHammer protection (preventive refreshes), respectively, for future DRAM chips with increased density and RowHammer vulnerability.

==> 17_appsecurityproof.tex <==
\section{Appendix II: Detailed Security Analysis for PARA}
\label{sec:app_revisitingpara}

\head{Threat Model} We assume a comprehensive {RowHammer} threat model,\cqlabel{CQ4} similar to {that assumed by} state-of-the-art works~\cite{kim2014flipping, park2020graphene, yaglikci2021blockhammer}, in which the attacker can 1)~fully utilize memory bandwidth, 2)~precisely time each memory request, and 3)~comprehensively and accurately know details of the memory controller and the DRAM chip. We do not consider any hardware or software component to be trusted or safe except {we assume that the DRAM commands issued by the memory controller are performed within the DRAM chip as intended.}


\head{PARA-Legacy} \agyarb{In this analysis we refer to the original design of PARA}~\cite{kim2014flipping} \agyarb{as \emph{PARA-Legacy}. PARA-Legacy} {configures} PARA's probability threshold (\gls{pth}), assuming {that} the attacker hammers an aggressor row {\emph{only enough times, but no more}}.
{With} more than an order of magnitude decrease in {the} {RowHammer threshold} in the last decade\cite{kim2020revisiting, frigo2020trrespass, hassan2021utrr, orosa2021deeper, yaglikci2022understanding}, \agyarb{it is possible for a memory access pattern to reach a hammer count as large as the RowHammer threshold 144 times} {within a refresh window of \SI{64}{\milli\second}},\footnote{{\Gls{hcfirst} for modern DRAM chips is as low as 9600~\cite{kim2020revisiting}. Assuming a \gls{trc} of \SI{46.25}{\nano\second}, performing 9600 row activations can be completed \emph{only} in \SI{444}{\micro\second}, which is 1/144.14 of a nominal refresh window of \SI{64}{\milli\second}. {As such, an attacker can perform 9600 activations for 144 times within a \SI{64}{\milli\second} refresh window.}}}
{requiring {a} revisit {of PARA's configuration methodology}.\footnote{A concurrent work also revisits PARA's configuration methodology~\cite{saroiu2022configure}.}}

\head{Our Approach in High Level}
\figref{fig:app_para_fsm} shows the probabilistic state machine that we use to 
calculate the {hammer count, which we define as the number of aggressor row activations} that may affect a victim row during a RowHammer attack.
Initially the {hammer count} is zero (state~0). When an {aggressor row} {is} activat{ed}, PARA {triggers a \emph{preventive} refresh with a probability of $\pth{}$. Since there are two rows that are adjacent to the activated row, PARA} refreshes {the} victim row with a probability of $\pth{}/2$, {in which case the {hammer} count is reset.} {Therefore,} the {hammer} count {{is incremented} with a probability of $1-\pth{}/2$ upon an {aggressor row} activation}. A \agyarb{memory access pattern is considered to be \emph{a successful RowHammer access pattern} when} {the hammer count} reaches the RowHammer threshold {($N_{RH}$)} within a \glsfirst{trefw}. 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/hira_fig9_low.pdf}
    \caption{Probabilistic state machine of {hammer} count in a PARA-protected system}
    \label{fig:app_para_fsm}
\end{figure}

{Because the time delay between two row activations targeting the same {bank} \emph{cannot} be smaller than \gls{trc}, an} attacker can perform {a maximum of} $\trefw{}/\trc{}$ state transitions within a \gls{trefw}. 
To account for all possible access patterns, we model a \emph{successful RowHammer {access pattern}} as a set of failed attempts (i.e., the victim row is refreshed before the {hammer} count reaches {the} RowHammer threshold), followed by a successful attempt {(i.e., the victim row is {\emph{not}} refreshed until the {hammer} count reaches {the} RowHammer threshold)}. {To {calculate} \gls{pth}{,} we follow a {five-}step approach. First, we calculate the probability of a failed attempt ($p_f$) and a successful attempt. Second, we calculate {the probability of observing a number ($N_f$) of consecutive failed attempts.}Third, we calculate
{\emph{the {overall} RowHammer success probability ($p_{RH}$)} as the overall probability of {\emph{all} possible successful RowHammer access patterns.}}
Fourth, we extend the probability calculation to account for \gls{trrslack}. Fifth, we calculate \gls{pth} for a given failure probability target.}

\head{{Step {1}: Failed and successful attempts}}
\expref{exp:app_failedattempt} {shows} $p_{f}(HC)$: the probability of a {\emph{failed} attempt with a given hammer count ($HC$). The attempt contains 1)~$HC$ consecutive aggressor row activations that do \emph{not} trigger a preventive} refresh, $(1-\pth{}/2)^{HC}$, {where $HC$ is smaller than the RowHammer threshold ($N_{RH}$)}, {and 2)~}an {aggressor row} activation {that triggers} a {preventive} refresh $(\pth{}/2)$.


\equ{p_{f}(HC) = (1-\pth{}/2)^{HC}\times\pth{}/2,~where~1\leq HC<N_{RH}}{exp:app_failedattempt}

{Similarly, we calculate the probability of a \emph{successful} attempt which has $N_{RH}$ consecutive aggressor row activations that do \emph{not} trigger a preventive refresh {as} $(1-p_{th}/2)^{N_{RH}}$.}


\head{{Step {2}: {The probability of} ${\bm{N_f}}$ {consecutive} failed attempts}}
{{Since a failed attempt may have a hammer count value in the range $[1, N_{RH})$, we account} for all possible hammer count {values} that {a failed attempt might have}.}
{\expref{exp:app_nconsecutivefailedattempts} shows the probability of {a given number of (}$N_f${)} consecutive failed attempts.}
\equ{\prod_{i=1}^{N_{f}} p_f(HC_i)=\prod_{i=1}^{N_{f}}((1-\pth{}/2)^{HC_i}\times\pth{}/2)~, where~1\leq HC_{i} < \hcfirst{}}{exp:app_nconsecutivefailedattempts}
    


\head{{Step 3: {Overall} RowHammer success probability}}
{To find the overall RowHammer success probability, we 1)~calculate the probability of the \emph{successful RowHammer access pattern which consists of $N_f$ consecutive failed attempts and one successful attempt ($p_{success}(N_{f})$)} for each possible value that $N_f$ can take and 2)~sum up the probability of all possible successful RowHammer access patterns: $\sum{p_{success}(N_f)}$.}
To do so, {we} multiply \expref{exp:app_nconsecutivefailedattempts} with the probability of a successful attempt: $(1-p_{th}/2)^{N_{RH}}$.
{\expref{exp:app_successfulattack}} shows {how we calculate $p_{success}(N_{f})$.} We derive \expref{exp:app_successfulattack} by evaluating the product on both terms in \expref{exp:app_nconsecutivefailedattempts}: $p_{th}/2$ and $(1-p_{th}/2)^{HC_i}$.




\equ{p_{success}(N_{f}) = (1-{\pth{}}/{2})^{\sum_{i=1}^{N_{f}} {HC_{i}}} \times ({\pth{}}/{2})^{N_{f}} \times (1-{\pth{}}/{2})^{\hcfirst{}}}{exp:app_successfulattack}

To account for the worst-case, we maximize 
$p_{success}(N_{f})$ {by choosing} the worst possible value for each $HC_{i}$ {value}. \textbf{Intuitively}, {the number of activations in a failed attempt should be minimized. Since} a failed attempt {has to perform at least one activation,
we conclude that all failed attempts} fail after only one row activation in the worst case. 
\textbf{Mathematically,} {our goal is} to maximize $p_{success}(N_{f})$. {{Since} $\pth{}$ is a value between zero and one,} we minimize the term $\sum_{i=1}^{N_{f}} {HC_{i}}$ to maximize $p_{success}(N_{f})$. Thus, we derive \expref{exp:app_prhn} {by choosing $HC_i=1$ to achieve} {the maximum (worst-case) $p_{success}(N_{f})$.}

\equ{
p_{success}(N_{f}) = (1-{\pth{}}/{2})^{N_{f}+\hcfirst{}} \times ({\pth{}}/{2})^{N_{f}}}{exp:app_prhn}

{{\expref{exp:app_prh}} shows {{the overall} RowHammer success probability} ($p_{RH}$), as the sum of all possible $p_{success}(N_f)$ values.}
{$N_{f}$ can be as small as 0 if {the} RowHammer attack does \emph{not} include any failed attempt and as large as} the maximum number of failed attempts that can fit in a refresh window {(\gls{trefw}) {together with a successful attempt}}.
Since $HC_i=1$ in the worst case, each failed attempt {costs only two row} activations ($2\times\trc{}$){:} {one aggressor row activation and one activation for preventively refreshing the victim row}. Thus, the execution time of $N_{f}$ {failed} attempts, {followed by one successful attempt is} $(2N_{f}+\hcfirst{})\times\trc{}$. {Therefore,} the maximum {value $N_{f}$ can take within a refresh window (\gls{trefw})} is ${N_{f}}_{max} = ((\trefw{}/\trc{})-\hcfirst{})/2$.

\equ{p_{RH} = \sum_{N_{f}=0}^{{N_{f}}_{max}} p_{success}(N_{f}),~~~{N_{f}}_{max} = (\trefw{}/\trc{}-\hcfirst{})/2}{exp:app_prh}

Using {\expsref{exp:app_prhn}} and~\ref{exp:app_prh}, we compute the {{overall} RowHammer success probability} for a given {PARA} probability threshold ($p_{th}$). 


\head{{Step 4: Accounting for \gls{trrslack}}}
The original PARA proposal~\cite{kim2014flipping} performs a {preventive} refresh immediately after the activated row is closed. However, \gls{hirasched} allows a {preventive} refresh to be queued {for a time window as long as \gls{trrslack}}. {Since the aggressor rows can be activated while a preventive refresh request is queued, we update {~\expsref{exp:app_prhn}} and~\ref{exp:app_prh}, assuming the worst case, where an aggressor row is activated as many times as possible {within \gls{trrslack} ({i.e.,} the maximum amount of time} the preventive refresh is queued).}
To do so, we {update} \expref{exp:app_prh}: {we reduce} {the RowHammer threshold ($N_{RH}$)} by {\gls{hcdeadline}}. Thus, we calculate ${N_{f}}_{max}$ and $\prh{}$ as shown in \expsref{exp:app_nmax} and~\ref{exp:app_prhdl}, respectively. 

\begin{equation}\footnotesize
{N_{f}}_{max} = ((\trefw{}/\trc{})-\hcfirst{}-{\hcdeadline{}})/2
\label{exp:app_nmax}
\end{equation}

\equ{p_{RH} = \sum_{N_{f}=0}^{{N_{f}}_{max}} (1-{\pth{}}/{2})^{{N_{f}}+\hcfirst{}-{\hcdeadline{}}} \times ({\pth{}}/{2})^{N_{f}}}{exp:app_prhdl}



\head{{Step 5: Finding $\bf{p_{th}}$}}
{We iteratively evaluate \expsref{exp:app_nmax} and \ref{exp:app_prhdl} to find} \gls{pth} for a {target} {{overall} RowHammer success probability of {$10^{-15}$}, as a typical consumer memory reliability target {(see, e.g.,~\cite{cai2012error, cai2017flashtbd, jedec2011failure, luo2016enabling, patel2017reaper, yaglikci2021blockhammer, kim2020revisiting, micheloni2015apparatus})}}.

\subsubsection{{Results}}


{We refer to {the} original PARA work~\cite{kim2014flipping} as PARA-Legacy. PARA-Legacy calculates {{the overall} RowHammer success probability} as ${p_{RH_{Legacy}}=(1-p_{th}/2)^{N_{RH}}}$ with an optimistic assumption that the attacker hammers an aggressor row \emph{only enough times, but no more}. To mathematically compare {{the overall} RowHammer success probability} that we calculate ($p_{RH}$) with $p_{RH_{Legacy}}$, we reorganize \expref{exp:app_prhdl}, which already includes ${p_{RH_{Legacy}}=(1-p_{th}/2)^{N_{RH}}}$, and derive \expref{exp:app_prhdiff}.}

\equ{
p_{RH} =k \times p_{RH_{Legacy}},~where~k = (1-\frac{\pth{}}{2})^{-{\hcdeadline}}\sum_{N_{f}=0}^{{N_{f}}_{max}}(\frac{\pth{}}{2}(1-\frac{\pth{}}{2}))^{{N_{f}}}
}{exp:app_prhdiff}

{
\expref{exp:app_prhdiff} shows that $p_{RH}$ {is a multiple of} $p_{RH_{Legacy}}$ by a factor of $k$, {where $k$ depends on a given system's properties (e.g., $N_{f_{max}}$)} and PARA's configuration (e.g., \gls{pth}).
{To understand the difference between $p_{RH}$ and $p_{RH_{Legacy}}$, we evaluate \expref{exp:app_prhdiff} for different RowHammer threshold values.\footnote{{We calculate for $N_{RefSlack}=0$, $t_{REFW}=64ms$, and $t_{RC}=46.25ns$.}}}
For {old DRAM chips (manufactured in} 2010-2013)~\cite{kim2014flipping}, $k$ is 1.0005 {(for $N_{RH}=50K$ and $p_{th}=0.001$~\cite{kim2014flipping})}, causing \emph{only} \SI{0.05}{\percent} variation in PARA's reliability target. {However,for future DRAM chips with $N_{RH}$ values of 1024 and 64 {($p_{th}$ values of 0.4730 and 0.8341)}, $k$ becomes 1.0331 and 1.3212, respectively. Therefore, the difference between {the two probabilities, $p_{RH}$ and $p_{RH_{Legacy}}$,} significantly increases as RowHammer worsens.}}
